SummIt: Iterative Text Summarization via ChatGPT

Text summarization systems have made significant progress in recent years, but typically generate summaries in one single step. However, the one-shot summarization setting is sometimes inadequate, as the generated summary may contain hallucinations or overlook essential details related to the reader's interests. This paper addresses this limitation by proposing SummIt, an iterative text summarization framework based on large language models like ChatGPT. Our framework enables the model to refine the generated summary iteratively through self-evaluation and feedback, resembling humans' iterative process when drafting and revising summaries. Furthermore, we explore the potential benefits of integrating knowledge and topic extractors into the framework to enhance summary faithfulness and controllability. We automatically evaluate the performance of our framework on three benchmark summarization datasets. We also conduct a human evaluation to validate the effectiveness of the iterative refinements and identify a potential issue of over-correction.

==> tables/context_num.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabular}{c|cccc|cccc}
\hline
\multirow{2}{*}{\textbf{Context \#}} & \multicolumn{4}{c|}{\textbf{Summarizer}} & \multicolumn{4}{c}{\textbf{Evaluator}} \Tstrut\Bstrut\\ \cline{2-9}
                             & \textbf{R1}   & \textbf{R2}   & \textbf{RL}   & \textbf{G-Score} & \textbf{R1}    & \textbf{R2}   & \textbf{RL}   & \textbf{G-Score} \Tstrut\Bstrut\\
\hline
\rowcolor{gray!10}
\multicolumn{9}{c}{\textbf{\textsl{CNN/DM}}} \Tstrut\Bstrut\\ \hline
1                            & 23.61 & 6.06 & 17.63 & \textbf{4.30} & 23.42 & 5.00 & 17.05 & \textbf{4.22} \Tstrut\\
2                            & \textbf{25.78} &\textbf{ 7.28} & \textbf{19.22} & 4.21 & 25.40 & \textbf{8.12} & 19.22 & 4.14 \\
3                            & 24.48 & 5.85 & 18.02 & 4.23 & \textbf{26.90} & 7.18 & \textbf{20.22} & 4.12 \\
4                            & 24.63 & 6.30 & 18.87 & 4.25 & 24.31 & 6.74 & 18.64 & 4.18 \\
5                            & 24.09 & 6.81 & 18.17 & 4.29 & 25.70 & 6.91 & 19.66 & 4.10 \\ \hline
\rowcolor{gray!10}
\multicolumn{9}{c}{\textbf{\textsl{XSum}}} \Tstrut\Bstrut\\ \hline
1                            & 17.89 & 3.72 & 14.02 & \textbf{4.33} & \textbf{18.84} & \textbf{4.68} & \textbf{14.72} & 4.12 \Tstrut\\
2                            & 16.98 & 3.95 & 12.88 & 4.22 & 18.83 & 3.11 & 14.68 & 4.13 \\
3                            & 18.30 & \textbf{4.85} & 13.99 & 4.32 & 16.32 & 3.65 & 12.53 & 4.16 \\
4                            & 17.21 & 3.83 & 13.37 & 4.23 & 17.35 & 3.41 & 12.80 & \textbf{4.25} \\
5                            & \textbf{19.43} & 4.84 & \textbf{14.38} & 4.08 & 15.56 & 4.12 & 12.70 & 4.24 \\ \hline
\end{tabular}
\caption{In-context learning experimental results on CNN/DM and XSum datasets of both summarizer and evaluator. For each dataset, we randomly sampled 50 data from the test set. Context \# is the number of context we feed into the summarizer and the evaluator.}
\label{context_num}
\end{table*}


==> tables/faithful.tex <==
\begin{table*}[ht]
\centering
\small
\scalebox{1}{
\begin{tabular}{c|ccccc|ccccc}
\hline
\multirow{2}*{} & \multicolumn{5}{c|}{\textbf{CNN/DM}} & \multicolumn{5}{c}{\textbf{XSum}} \Tstrut \Bstrut\\ \cline{2-11}
                      & \textbf{R1}    & \textbf{R2}    & \textbf{RL}  & \textbf{GPT-Eval} & \textbf{FactCC} &\textbf{R1}   & \textbf{R2}   & \textbf{RL}  & \textbf{GPT-Eval} & \textbf{FactCC} \Tstrut \Bstrut\\ \hline

ChatGPT-Init               & 39.44 & 16.14 & 29.83 & 3.46 & 56.29 & 21.61 & 5.98 & 17.60 & 3.47 & 28.00 \Tstrut\\
ChatGPT-Final              & 36.50 & 13.49  & 26.76 & 4.33 & 68.35 & 21.92 & 5.93 & 17.62 & 4.24 & 36.00 \Bstrut\\ \hline

\hline

OpenIE-Init & 41.04 & 18.86 & 32.20 & 3.87 & 59.83 & 22.01 & 5.11 & 17.06 & 3.85 & 51.68 \Tstrut \\
OpenIE-Final & 34.36 & 14.05 & 26.40 & 4.92 & 49.70 & 19.72 & 3.85 & 15.36 & 4.95 & 47.24 \Bstrut\\ \hline
\end{tabular}
}
\caption{Experimental results of providing the relationships extracted by OpenIE to ChatGPT.}
\label{faithful_full}
\end{table*}


% ChatGPT-Init               & 36.01 & 12.82 & 26.13 & 3.58 & 10.23 & 21.20 & 5.51 & 17.38 & 3.64 & 11.86  \Tstrut\\
% ChatGPT-Final              & 27.50 & 7.65  & 19.37 & 4.32 & 15.69 & 17.10 & 4.01 & 14.11 & 4.38 & 14.41  \Bstrut\\ 
% \hline

==> tables/incontext.tex <==
\begin{table*}[h]
\centering
\small
\scalebox{1}{
\begin{tabular}{c|cccc|cccc}
\hline
\multirow{2}*{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{CNN/DM}} & \multicolumn{4}{c}{\textbf{XSum}} \Tstrut \Bstrut\\ \cline{2-9}
                      & \textbf{R1}    & \textbf{R2}    & \textbf{RL}  & \textbf{GPT-Eval} & \textbf{R1}   & \textbf{R2}   & \textbf{RL}  & \textbf{GPT-Eval} \Tstrut \Bstrut\\ \hline
                      
ChatGPT-Init               & 39.44 & 16.14 & 29.83 & 3.46 & 21.61 & 5.98 & 17.60 & 3.47  \Tstrut\\
ChatGPT-Final              & 36.50 & 13.49  & 26.76 & 4.33  & 21.92 & 5.93 & 17.62 & 4.24 \Bstrut\\ \hline
In-context-Init               & \textbf{40.00} & \textbf{16.39} & \textbf{30.02} & 3.57  & \textbf{23.96} & \textbf{7.36} & \textbf{19.36} & 3.57 \Tstrut\\
In-context-Final              & 37.29 & 13.60  & 26.87 & \textbf{4.35}  & 22.04 & 6.20 & 17.46 & \textbf{4.32}  \Bstrut\\ 
\hline
\end{tabular}
}

\caption{In-context learning experiment results on 1000 test samples. In-context-Init and In-context-Final represent the summary generated by ChatGPT with in-context learning.}
\label{incontext}
\end{table*}

==> tables/intra_human_eval.tex <==
% \begin{table}[ht]
% \centering
% \small
% \begin{tabular}{c|cc}
% \hline
%            & \textbf{Improved}     & \textbf{Follow Inst}    \Tstrut\Bstrut\\ \hline
% CNN/DM & 0.65 & 0.89 \Tstrut\\
% XSum    & 0.53  & 0.91    \Bstrut\\
% \hline
% \end{tabular}
% \caption{Human evaluation to justify the refinement behavior of SummIt. The column 'Improved' indicates when iterative refinement improved summaries as per human evaluators. The column 'Follow Inst' shows the ratio of refined summaries that follows the evaluator's evaluation reationale.}
% \label{tab:intra_eval}
% \end{table}

\begin{table*}[ht]
\centering
\small
\scalebox{0.95}{
\begin{tabular}{c|cc|cc|cc|cc}
\hline
\multirow{2}*{}  & \multicolumn{2}{c|}{\textbf{Iter 2}} & \multicolumn{2}{c|}{\textbf{Iter 3}} & \multicolumn{2}{c|}{\textbf{Iter 4}} & \multicolumn{2}{c}{\textbf{Iter 5}} \Tstrut \Bstrut\\ \cline{2-9}

~ & \textbf{Improved} & \textbf{Follow Inst} & \textbf{Improved} & \textbf{Follow Inst} &  \textbf{Improved} & \textbf{Follow Inst} &  \textbf{Improved} & \textbf{Follow Inst} \Tstrut \Bstrut\\ \hline

\textbf{CNN/DM} & \textbf{0.82} & \textbf{0.96} & 0.62 & \textbf{0.96} & 0.53 & 0.92 & 0.48 & 0.94 \Tstrut\\

\textbf{XSum} &\textbf{0.84} & \textbf{0.98} & 0.54 & 0.94 & 0.55 & 0.92 & 0.46 & 0.92 \\
% CNN/DM & 0.65 & 0.89 \Tstrut\\
% XSum    & 0.53  & 0.91    \Bstrut\\
\hline
\end{tabular}
}
\caption{Human evaluation to justify the refinement behavior of SummIt. The column 'Improved' indicates when iterative refinement improved summaries as per human evaluators. The column 'Follow Inst' shows the ratio of refined summaries that follows the evaluator's evaluation rationale. \textcolor{red}{change table into line plot}}
\label{tab:intra_eval}
\end{table*}

==> tables/res.tex <==
\begin{table*}[t]
\centering
\scalebox{1.0}{
\begin{tabular}{l@{\hspace{0.8\tabcolsep}}|c|cccc}
\hline
{\textbf{Datasets}} & Models & R-1  & R-2 & R-L & R-Lsum  \\
\hline
%\multirow{2}{*}{\textit{AQuaMuse}} & \textit{Fine-tuning} & $-$ & $-$ & $-$ & $-$ & $-$\\
%& \textit{ChatGPT} & $\textbf{-} $ & $\textbf{-} $ & $\textbf{-} $ & $-$ & $-$\\
%\hline  
\multirow{2}{*}{\textit{CovidET}} & \textit{Fine-tuning} & $\textbf{26.19}$ &$\textbf{6.85}$ & $\textbf{17.86}$ & $\textbf{20.82}$ \\
& \textit{ChatGPT}  & $20.81 $ & $3.99 $ & $15.35$ & $15.36$ \\
\hline
\multirow{2}{*}{\textit{NEWTS}} & \textit{Fine-tuning} & $31.78$ & $10.83$ & $20.54$ & $-$ \\
& \textit{ChatGPT} & $\textbf{32.54}$ & $\textbf{11.37} $ & $\textbf{20.74}$ & $20.74 $ \\
\hline
\multirow{2}{*}{\textit{QMSum}} & \textit{Fine-tuning} & $\textbf{32.29}$ & $8.67$ & $\textbf{28.17}$ & $-$\\
& \textit{ChatGPT} & $28.34$ & $\textbf{8.74}$ & $17.81 $ & $18.01$\\
\hline
\multirow{2}{*}{\textit{QMSum(Golden)}} & \textit{Fine-tuning} & $36.06$ & $11.36$ & $\textbf{31.27}$ & $-$\\
& \textit{ChatGPT} & $\textbf{36.83} $ & $\textbf{12.78}$ & $24.23$ & $ 24.19 $   \\
\hline
\multirow{2}{*}{\textit{SQuaLITY}} & \textit{Fine-tuning} & $\textbf{38.20}$ & $\textbf{9.00}$ & $\textbf{20.20}$ & $-$ \\
& \textit{ChatGPT} & $37.02 $ & $8.19$ & $18.45$ & $22.56$ \\
\hline
 \multirow{2}{*}{\textit{Avg.}} & \textit{Fine-tuning} & $\textbf{32.90}$ & $\textbf{9.34}$ & $\textbf{23.61}$ & $-$ \\
& \textit{ChatGPT} & $30.94$ & $8.96 $ & $19.22 $ & $-$  \\
\hline
\end{tabular}
}
\caption{ Comparison between ChatGPT zero-shot performance with previous Fine-tuning(FT) results.}
\label{tab:res}
\end{table*}



==> tables/res_1000.tex <==
\begin{table*}[ht]
\vspace{-12pt}
\centering
\small
\begin{tabular}{c | c c c c| c c c c}
\hline \multirow{2}*{\# Context} & \multicolumn{4}{c|}{{CNN/DM}} & \multicolumn{4}{c}{{XSum}} \Tstrut\Bstrut\\
\cline{2-9}
~ & {R1} & {R2} & {RL} & {BERTScore} & {R1} & {R2} & {RL} & {BERTScore} \Tstrut\Bstrut\\
\hline
0 & 39.25 & 17.09 & 25.64 & 0.87 & 19.85 & \textbf{2.96} & 13.29 & 0.84 \Tstrut\\
3 & 38.62 & 16.35 & 25.25 & 0.86 & \textbf{19.86} & 2.92 & 13.22 & \textbf{0.84} \\
3 w/o r & \textbf{40.10} & \textbf{17.80} & \textbf{25.95} & \textbf{0.87} & 19.31 & 2.67 & 13.15 & 0.84 \Bstrut\\
\hline
\end{tabular}
\caption{Experimental results on CNN/DM and XSum datasets. We ran our experiment on 1000 test data randomly sampled from two datasets. 3 w/o r represents 3 context documents-summary pairs without reason are given to the model}
\label{exp_result}
\end{table*}

==> tables/res_stats.tex <==
\begin{table*}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{l@{\hspace{0.8\tabcolsep}}|c|ccccccc}
\hline
{\textbf{Datasets}} & Text & U-1-gram  & U-2-gram & U-3-gram & U-4-gram & Coverage & Density & Compression \\
\hline 
\multirow{2}{*}{\textit{CovidET}} & \textit{Reference} & $0.59$ & $0.95$ & $0.99$ & $0.99$ & $0.60$ & $0.90$ & $11.84$ \\
& \textit{ChatGPT}  & $0.42$ & $0.86$ & $0.97$ & $0.99$ & $0.66$ & $1.19$ & $6.92$ \\
\hline
\multirow{2}{*}{\textit{NEWTS}} & \textit{Reference} & $0.30$ & $0.69$ & $0.84$ & $0.90$ & $0.78$ & $2.84$ & $9.66$ \\
& \textit{ChatGPT} & $0.15$ & $0.50$ & $0.69$ & $0.81$ & $0.89$ & $4.13$ & $4.03$ \\
\hline
\multirow{2}{*}{\textit{QMSum}} & \textit{Reference} & $0.19$ & $0.65$ & $0.88$ & $0.96$ & $0.87$ & $2.15$ & $99.76$ \\
& \textit{ChatGPT} & $0.26$ & $0.73$ & $0.89$ & $0.95$ & $0.84$ & $1.97$ & $44.86$ \\
\hline
\multirow{2}{*}{\textit{QMSum(Golden)}} & \textit{Reference} & $0.29$ & $0.69$ & $0.88$ & $0.95$ & $0.77$ & $2.05$ & $15.68$ \\
& \textit{ChatGPT} & $0.26$ & $0.66$ & $0.85$ & $0.93$ & $0.79$ & $2.15$ & $10.74$ \\
\hline
\multirow{2}{*}{\textit{SQuaLITY}} & \textit{Reference} & $0.25$ &$0.85$ & $0.97$ & $0.99$ & $0.83$ & $1.55$ & $32.57$ \\
& \textit{ChatGPT} & $0.33$ & $0.82$ & $0.93$ & $0.97$ & $0.81$ & $1.81$ & $24.83$ \\
\hline

\end{tabular}
}
\caption{ Comparison between ChatGPT zero-shot performance with references on various metrics. U-1/2/3/4-gram represents unique 1/2/3/4 gram.}
\label{tab:res_stats}
\end{table*}



==> tables/stats.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c|c|c|c|c|c }
        % \hline
        \toprule
        \textbf{Type} & \textbf{Dataset} & \textbf{Domain} & \#\textbf{Input Tk.} &\#\textbf{Output Tk.} & \#\textbf{Asp. Type}  \\
        \hline
        \multirow{2}{*}{Query}
        & QMSum \cite{zhong-etal-2021-qmsum} & Meeting & 9,070(2,505*) & 70 & 1,566  \\
        & SQuALITY \cite{wang2022squality} & Story & 6,052 & 252 & 437   \\
        \hline
        \multirow{2}{*}{Aspect}
        & CovidET \cite{zhan2022you}  & Reddit &  192 & 27 & 7  \\
        & NEWTS \cite{bahrainian-etal-2022-newts}  & News & 602 & 74 & 50 \\

        \bottomrule
    \end{tabular}
    }
    \caption{
    Statistics of the query/aspect-based summarization datasets that we used.
    \#\textbf{Input Tk.} and \#\textbf{Output Tk.} represent the number of input and output token lengths, respectively. \#\textbf{Asp. Type} is the number of all aspect types. 2,505* represents the average token number in golden inputs.
    }
    \label{tab:big_table}
\end{table*}


